Free quantum analogue of Coxeter group $D_4$

We define the quantum group $D_4^+$ -- a free quantum version of the demihyperoctahedral group $D_4$ (the smallest representative of the Coxeter series $D$). In order to do so, we construct a free analogue of the property that a $4\times4$ matrix has determinant one. Such analogues of determinants are usually very hard to define for free quantum groups in general and our result only holds for the matrix size $N=4$. The free $D_4^+$ is then defined by imposing this generalized determinant condition on the free hyperoctahedral group $H_4^+$. Moreover, we give a detailed combinatorial description of the representation category of $D_4^+$.

==> graphmor.tex <==
\def\Gid{\Graph{
\GS 0/1:1/;
\GV 0.5:1;
}}

\def\Gpair{\Graph{
\GS 0.3/0.5:1/1.5,2/1.5;
\GS 0.3/0:1/,2/;
\GV 0.5:1.5;
}}

\def\Guppair{\Graph{
\GS 0.7/0.5:1/1.5,2/1.5;
\GS 0.7/1:1/,2/;
\GV 0.5:1.5;
}}

\def\Gconnecter{\Graph{
\GS 0.7/0.5:1/1.5,2/1.5;
\GS 0.3/0.5:1/1.5,2/1.5;
\GS 0.7/1:1/,2/;
\GS 0.3/0:1/,2/;
\GV 0.5:1.5;
}}

\def\GEconnecter{\Graph{
\GE 0.7/0.5:1/1.5,2/1.5;
\GE 0.3/0.5:1/1.5,2/1.5;
\GS 0.7/1:1/,2/;
\GS 0.3/0:1/,2/;
\GV 0.5:1.5;
\GV 0.3:1,2;
\GV 0.7:1,2;
}}

\def\Gfork{\Graph{
\GS 0.3/0.5:1/1.5,2/1.5;
\GS 0.5/1:1.5/;
\GS 0.3/0:1/,2/;
\GV 0.5:1.5;
}}

\def\Gmerge{\Graph{
\GS 0.7/0.5:1/1.5,2/1.5;
\GS 0.7/1:1/,2/;
\GS 0.5/0:1.5/;
\GV 0.5:1.5;
}}

\def\Gfour{\Graph{
\GS 0.3/0.5:1/2.5,2/2.5,3/2.5,4/2.5;
\GS 0.3/0:1/,2/,3/,4/;
\GV 0.5:2.5;
}}

\def\Gcross{\Graph{
\GS 0/1:1/2,2/1;
\GV 0.75:1.25,1.75;
}}

\def\Ggrpth{\Graph{
\GV 0.5:2;
\GV 0.8:1.4;
\GS 0.5/1:2/2,2/3;
\GS 0.5/0:2/1,2/2;
\GS 0.8/1:1.4/1;
\GS 0.2/0:2.6/3;
\GSa (1.4,0.8) (-0.6,0.3) (0.25,0.25)
}}

\def\GA{\Graph{
\GE 0.25/0.75:1/;
\GS 0/0.25:1/;
\GS 0.75/1:1/;
\GV 0.25:1;
\GV 0.75:1;
}}

\def\GAA{\Graph{
\GE 0.25/0.75:1.15/;
\GE 0.25/0.75:0.85/;
\GS 0/0.25:1/;
\GS 0.75/1:1/;
\GV 0.25:1;
\GV 0.75:1;
}}


\def\Graph#1{%
\ifmmode
\mathchoice{
\,\GraphA{0.25em}{1em}{1em}{#1}\,%
}{
\,\GraphA{0.25em}{0.7em}{1em}{#1}\,%
}{
\,\GraphA{0.175em}{0.55em}{0.7em}{#1}\,%
}{
\,\GraphA{0.125em}{0.4em}{0.5em}{#1}\,%
}\else%
\thinspace\GraphA{0.25em}{0.7em}{1em}{#1}\thinspace%
\fi%
}

\def\GraphA#1#2#3#4{%
\pgfpicture
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
#4
\endpgfpicture
}

\def\GSA#1#2#3/#4,{\ifx,#3,\else%
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\ifx,#4,\pgfpathlineto{\pgfpointxy{#3}{#2}}
\else   \pgfpathlineto{\pgfpointxy{#4}{#2}}\fi
\pgfusepath{stroke}
\fihere\GSA{#1}{#2}\fi}

\def\GS#1/#2:#3;{%
\GSA{#1}{#2}#3,/,
}

\def\GSa (#1,#2) (#3,#4) (#5,#6){%
\pgfpathmoveto{\pgfpointxy{#1}{#2}}
\pgfpatharcaxes{0}{180}{\pgfpointxy{#3}{#4}}{\pgfpointxy{#5}{#6}}
\pgfusepath{stroke}
}

\def\GEa (#1,#2) (#3,#4) (#5,#6){%
\pgfsetlinewidth{2.5\pgflinewidth}
\pgfpathmoveto{\pgfpointxy{#1}{#2}}
\pgfpatharcaxes{0}{180}{\pgfpointxy{#3}{#4}}{\pgfpointxy{#5}{#6}}
\pgfusepath{stroke}
\pgfsetlinewidth{0.4\pgflinewidth}
}

%\definecolor{adjcol}{rgb}{0.2,0.2,0.6}

\def\GE#1/#2:#3;{%
\pgfsetlinewidth{2.5\pgflinewidth}
%\pgfsetstrokecolor{adjcol}
\GSA{#1}{#2}#3,/,
\pgfsetlinewidth{0.4\pgflinewidth}
%\pgfsetstrokecolor{black}
}

\def\GraphV#1#2{
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{0.1em}
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
}

\def\GVA#1#2,{\ifx,#2,\else%
\GraphV{#2}{#1}
\fihere\GVA{#1}\fi
}

\def\GV#1:#2;{%
\GVA{#1}#2,,
}

\def\GraphW#1#2{
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{0.1em}
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
}

\def\GWA#1#2,{\ifx,#2,\else%
\GraphW{#2}{#1}
\fihere\GWA{#1}\fi
}

\def\GW#1:#2;{%
\GWA{#1}#2,,
}


==> partmac.tex <==
%%Macro package for typeseting set partitions
%%Daniel Gromada 2019--2020
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%First, also as an example, we define shortcuts for some short partitions using word representation.

%%%Partitions with lower points only

%%k=1

\def\La{\LPartition{0.6:1}{}}

%%k=2

\def\Laa{\LPartition{}{0.6:1,2}}
\def\Lab{\LPartition{0.6:1,2}{}}

%k=3

\def\Laaa{\LPartition{}{0.6:1,2,3}}
\def\Laab{\LPartition{0.6:3}{0.6:1,2}}
\def\Laba{\LPartition{0.4:2}{0.8:1,3}}
\def\Labb{\LPartition{0.6:1}{0.6:2,3}}
\def\Labc{\LPartition{0.6:1,2,3}{}}

%k=4


\def\Laaaa{\LPartition{}{0.6:1,2,3,4}}
\def\Laaab{\LPartition{0.6:4}{0.6:1,2,3}}
\def\Laaba{\LPartition{0.4:3}{0.8:1,2,4}}
\def\Labaa{\LPartition{0.4:2}{0.8:1,3,4}}
\def\Labbb{\LPartition{0.6:1}{0.6:2,3,4}}
\def\Laabb{\LPartition{}{0.6:1,2;0.6:3,4}}
\def\Labba{\LPartition{}{0.8:1,4;0.4:2,3}}
\def\Labab{\LPartition{}{0.8:2,4;0.4:1,3}}
\def\Laabc{\LPartition{0.6:3,4}{0.6:1,2}}
\def\Labac{\LPartition{0.4:2,4}{0.8:1,3}}
\def\Labca{\LPartition{0.4:2,3}{0.8:1,4}}
\def\Labbc{\LPartition{0.6:1,4}{0.6:2,3}}
\def\Labcb{\LPartition{0.4:1,3}{0.8:2,4}}
\def\Labcc{\LPartition{0.6:1,2}{0.6:3,4}}
\def\Labcd{\LPartition{0.6:1,2,3,4}{}}

%%%Partitions with upper points only

%%k=1

\def\Ua{\UPartition{0.4:1}{}}

%%k=2

\def\Uaa{\UPartition{}{0.4:1,2}}
\def\Uab{\UPartition{0.4:1,2}{}}

%k=3

\def\Uaaa{\UPartition{}{0.5:1,2,3}}
\def\Uaab{\UPartition{0.4:3}{0.4:1,2}}
\def\Uaba{\UPartition{0.6:2}{0.2:1,3}}
\def\Uabb{\UPartition{0.4:1}{0.4:2,3}}
\def\Uabc{\UPartition{0.4:1,2,3}{}}

%k=4

\def\Uaaaa{\UPartition{}{0.4:1,2,3,4}}
\def\Uaaab{\UPartition{0.4:4}{0.4:1,2,3}}
\def\Uaaba{\UPartition{0.6:3}{0.2:1,2,4}}
\def\Uabaa{\UPartition{0.6:2}{0.2:1,3,4}}
\def\Uabbb{\UPartition{0.4:1}{0.4:2,3,4}}
\def\Uaabb{\UPartition{}{0.4:1,2;0.4:3,4}}
\def\Uabba{\UPartition{}{0.2:1,4;0.6:2,3}}
\def\Uabab{\UPartition{}{0.2:2,4;0.6:1,3}}
\def\Uaabc{\UPartition{0.4:3,4}{0.4:1,2}}
\def\Uabac{\UPartition{0.6:2,4}{0.2:1,3}}
\def\Uabca{\UPartition{0.6:2,3}{0.2:1,4}}
\def\Uabbc{\UPartition{0.4:1,4}{0.4:2,3}}
\def\Uabcb{\UPartition{0.6:1,3}{0.2:2,4}}
\def\Uabcc{\UPartition{0.4:1,2}{0.4:3,4}}
\def\Uabcd{\UPartition{0.4:1,2,3,4}{}}

%%%Partitions with same amount of upper and lower points

%%k=1, l=1

\def\Paa{\Partition{
\Pline (1,0) (1,1)
}}

\def\Pab{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:1
}}

%k=4

\def\Paaaa{\Partition{
\Pblock 0to0.3:1,2
\Pblock 1to0.7:1,2
\Pline (1.5,0.3) (1.5,0.7)
}}
\def\Paaab{\Partition{
\Pblock 1to0.7:1,2
\Psingletons 0to0.3:2
\Pline (1,0) (1,0.7)
}}
\def\Paaba{\Partition{
\Pblock 1to0.7:1,2
\Psingletons 0to0.3:1
\Pline (2,0) (2,0.7)
}}
\def\Pabaa{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:1
\Pline (2,0.3) (2,1)
}}
\def\Pabbb{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:2
\Pline (1,0.3) (1,1)
}}
\def\Paabb{\Partition{
\Pblock 0to0.3:1,2
\Pblock 1to0.7:1,2
}}
\def\Pabba{\Partition{
\Pline (1,0) (1,1)
\Pline (2,0) (2,1)
}}
\def\Pabab{\Partition{
\Pline (1,0) (2, 1)
\Pline (1,1) (2, 0)
}}
\def\Paabc{\Partition{
\Psingletons 0to0.3:1,2
\Pblock 1to0.7:1,2
}}
\def\Pabcc{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:1,2
}}
\def\Pabac{\Partition{
\Psingletons 0to0.3:2
\Psingletons 1to0.7:1
\Pline (1,0) (2,1)
}}
\def\Pabcb{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:2
\Pline (2,0) (1,1)
}}
\def\Pabca{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:1
\Pline (2,0) (2,1)
}}
\def\Pabbc{\Partition{
\Psingletons 0to0.3:2
\Psingletons 1to0.7:2
\Pline (1,0) (1,1)
}}
\def\Pabcd{\Partition{
\Psingletons 0to0.3:1,2
\Psingletons 1to0.7:1,2
}}

%k=6

\def\Pabcabc{\Partition{
\Pline (1,0) (3, 1)
\Pline (2,0) (2, 1)
\Pline (3,0) (1, 1)
}}
\def\Pabcabd{\Partition{
\Pline (1,0) (3, 1)
\Pline (2,0) (2, 1)
\Psingletons 0to0.3:3
\Psingletons 1to0.7:1
}}
\def\Pabcadc{\Partition{
\Pline (1,0) (3, 1)
\Pline (3,0) (1, 1)
\Psingletons 0to0.2:2
\Psingletons 1to0.8:2
}}
\def\Pabcdbc{\Partition{
\Pline (2,0) (2, 1)
\Pline (3,0) (1, 1)
\Psingletons 0to0.3:1
\Psingletons 1to0.7:3
}}
\def\Pabcade{\Partition{
\Pline (1,0) (3, 1)
\Psingletons 0to0.2:2,3
\Psingletons 1to0.8:1,2
}}
\def\Pabcdec{\Partition{
\Pline (3,0) (1, 1)
\Psingletons 0to0.2:1,2
\Psingletons 1to0.8:2,3
}}
\def\Pabcdbe{\Partition{
\Pline (2,0) (2, 1)
\Psingletons 0to0.3:1,3
\Psingletons 1to0.7:1,3
}}
\def\Pabcdef{\Partition{
\Psingletons 0to0.3:1,2,3
\Psingletons 1to0.7:1,2,3
}}

\def\Paabaab{\Partition{
\Pblock 1to0.75:2,3
\Pblock 0to0.25:1,2
\Pline (1.5,0.25)(2.5,0.75)
\Pline (3,0)(1,1)
}}

%%%Some aliases

%\def\singleton{{\mathord{\uparrow}}}
%\def\upsingleton{{\mathord{\downarrow}}}
\def\singleton{\LPartition{\Ps1:1}{}}
\def\upsingleton{\UPartition{\Ps0:1}{}}
\let\pairpart=\Laa
\let\uppairpart=\Uaa
\let\fourpart=\Laaaa
\let\idpart=\Paa
\let\disconnecterpart=\Pab
\let\connecterpart=\Paaaa
\let\crosspart=\Pabab
\let\positionerpart=\Pabcb
\let\halflibpart=\Pabcabc


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%The macros

\def\textchoice#1#2#3#4#5{\ifmmode\mathchoice{#1}{#2}{#3}{#4}\else #5\fi}
\def\fihere#1\fi{\fi#1}

%definition of the \Partition command
\def\Partition#1{\def\Ptmp{#1}%
\futurelet\nextchar\PartitionB
}

\def\BigPartition#1{\def\Ptmp{#1}%
\futurelet\nextchar\BigPartitionB
}

\def\PartitionD{%
\thinspace\textchoice
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}
{\PartitionA{0.175em}{0.55em}{0.7em}{\Ptmp}}
{\PartitionA{0.125em}{0.4em}{0.5em}{\Ptmp}}
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}%
\thinspace%
}

\def\BigPartitionD{%
\thinspace\textchoice
{\PartitionA{1em}{0.9em}{2.5em}{\Ptmp}}
{\PartitionA{0.75em}{0.7em}{2em}{\Ptmp}}
{\PartitionA{0.25em}{0.5em}{1em}{\Ptmp}}
{\PartitionA{0.20em}{0.4em}{0.8em}{\Ptmp}}
{\PartitionA{0.75em}{0.7em}{2em}{\Ptmp}}%
\thinspace
}

\newcount\tmpx
\newcount\tmpy
\def\PartitionB{\if[\nextchar\let\next=\PartitionC\else\let\next=\PartitionD\fi\next}
\def\BigPartitionB{\if[\nextchar\let\next=\BigPartitionC\else\let\next=\BigPartitionD\fi\next}
\def\PartitionC[#1]{\tmpx=0\tmpy=0\expandafter\def\expandafter\Ptmp\expandafter{\Ptmp\Ppointlist#1]}\PartitionD}
\def\BigPartitionC[#1]{\tmpx=0\tmpy=0\expandafter\def\expandafter\Ptmp\expandafter{\Ptmp\Ppointlist#1]}\BigPartitionD}

\def\Ppointlist#1{\advance\tmpx by 1\if#1]\else
	\csname P#1\endcsname(\the\tmpx,\the\tmpy)
	\fihere\Ppointlist\fi}

\def\Pwidth{0.05}

\def\PartitionA#1#2#3#4{%
\pgfpicture
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
\pgfsetlinewidth{\Pwidth em}
#4
\endpgfpicture
}

%\Pline, \Psingletons, \Pblock, \Ptext,...

\def\Pline(#1,#2)#3(#4,#5){
\pgfpathmoveto{\pgfpointxy{#1}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#5}}
\pgfusepath{stroke}
}

\def\Psingletons #1to#2:#3 {\PsingletonsA{#1}{#2}#3,,}
\def\PsingletonsA#1#2#3,{\ifx,#3,\else
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\pgfpathlineto{\pgfpointxy{#3}{#2}}
\pgfusepath{stroke}
\fihere\PsingletonsA{#1}{#2}\fi}

\def\Pblock #1to#2:#3 {\PblockA{#1}{#2}#3,,}
\def\PblockA#1#2#3,#4,{\ifx,#4,\else
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\pgfpathlineto{\pgfpointxy{#3}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#1}}
\pgfusepath{stroke}
\fihere\PblockA{#1}{#2}#4,\fi}

\def\Ptext(#1,#2)#3{%
\pgftext[at={\pgfpointxy{#1}{#2}}]{#3}
}

%\LPartition,\Upartition

\def\LPartition#1#2{\Partition{
\LPartitionB#2;;
\LPartitionA#1;;
}}

\def\LPartitionA#1;{\ifx;#1;\else
\Lsingletons #1 
\fihere\LPartitionA\fi}

\def\LPartitionB#1;{\ifx;#1;\else
\Pblock 0to#1 
\fihere\LPartitionB\fi}

\def\UPartition#1#2{\Partition{
\UPartitionB#2;;
\UPartitionA#1;;
}}

\def\UPartitionA#1;{\ifx;#1;\else
\Usingletons #1 
\fihere\UPartitionA\fi}

\def\UPartitionB#1;{\ifx;#1;\else
\Pblock 1to#1 
\fihere\UPartitionB\fi}

\def\Lsingletons #1#2 {%
	\ifcat\noexpand#1\noexpand\ \Ppoint0 #1#2 \else\Psingletons 0to#1#2 \fi
}
\def\Usingletons #1#2 {%
	\ifcat\noexpand#1\noexpand\ \Ppoint1 #1#2 \else\Psingletons 1to#1#2 \fi
}

%colors

\def\Pcolw{0.1}

\expandafter\def\csname P/\endcsname{\advance\tmpy by1 \tmpx=0}
\expandafter\def\csname P0\endcsname{}

\def\Pw (#1,#2){
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{\Pcolw em}
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
}

\def\Pb (#1,#2){
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{\Pcolw em}
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
}

\def\Ps#1(#2,#3){
	\pgfsetarrowsend{to}
	\pgfpathmoveto{\pgfpointxy{#2}{#3}}
	\pgfpathlineto{\pgfpointxy{#2}{#1}}
	\pgfusepath{stroke}
	\pgftransformreset
	\pgfsetarrowsend{}
}

\def\Pq (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	\pgfpathmoveto{\pgfpoint{-\Pcolw em}{-\Pcolw em}}
	\pgfpathlineto{\pgfpoint{-\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{-\Pcolw em}}
	\pgfpathclose
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
	\pgftransformreset
}

\def\PQ (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	\pgfpathmoveto{\pgfpoint{-\Pcolw em}{-\Pcolw em}}
	\pgfpathlineto{\pgfpoint{-\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{-\Pcolw em}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
	\pgftransformreset
}

\def\Lt (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfusepath{stroke}}
	\pgftransformreset
}
\def\Ut (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{-2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfusepath{stroke}}
	\pgftransformreset
}
\def\LT (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}}
	\pgftransformreset
}
\def\UT (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{-2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}}
	\pgftransformreset
}

\def\Ppoint #1 #2:#3 {\PpointA{#1}{#2}#3,,}
\def\PpointA#1#2#3,{\ifx,#3,\else #2(#3,#1)\fihere\PpointA{#1}{#2}\fi}

\def\coldefA #1 #2{\kern0.1ex\vcenter{\hbox{\def\Pcolw{#1}\pgfpicture#2(0,0)\endpgfpicture}}\kern0.1ex}

\def\coldef#1#2{\def#1{{\textchoice
{\coldefA 0.15 #2}{\coldefA 0.15 #2}{\coldefA 0.1 #2}{\coldefA 0.08 #2}{$\coldefA 0.15 #2$}}}}

\coldef\bcol\Pb
\coldef\wcol\Pw
\coldef\qcol\Pq
\coldef\Qcol\PQ
\coldef\tcol\Lt
\coldef\Tcol\LT

\def\singext{\LPartition{\Lt:1}{}}
\def\upsingext{\UPartition{\Ut:1}{}}
\def\idext{
	\Partition{
	\Lt (1,0)
	\Ut (1,1)
	}}
\def\positionerext{
	\Partition{
	\Lt (1,0)
	\Ut (2,1)
	\Pline(2,0)(1,1)
	}}
\def\globcolext{
	\Partition{
	\Lt (1,0)
	\Ut (3,1)
	\Pline(2,0)(1,1)
	\Pline(3,0)(2,1)
	}}

